Introducing k4.0s: a Model for Mixed-Criticality Container Orchestration in Industry 4.0 (extended)

Time predictable edge cloud is seen as the answer for many arising needs in Industry 4.0 environments, since it is able to provide flexible, modular, and reconfigurable services with low latency and reduced costs. Orchestration systems are becoming the core component of clouds since they take decisions on the placement and lifecycle of software components. Current solutions start introducing real-time containers support for time predictability; however, these approaches lack of determinism as well as support for workloads requiring multiple levels of assurance/criticality. In this paper, we present k4.0s, an orchestration model for real-time and mixed-criticality environments, which includes timeliness, criticality and network requirements. The model leverages new abstractions for both node and jobs, e.g., node assurance, and requires novel monitoring strategies. We sketch an implementation of the proposal based on Kubernetes, and present an experimentation motivating the need for node assurance levels and adequate monitoring.

==> 1_introduction_full.tex <==
 %\mb{IIoT e I4.0, necessità di orchestrazione in factory riconfigurabili, problemi attuali, carichi eterogenei, mixed crit -- 0.75}
%%% I4.0, IIoT, Fog/Edge computing
\mb{conservare intro, e tagliare prima colonna per rt-cloud}
In recent years, we are witnessing the increasing adoption of IT technologies in several industrial domains (e.g., railways, avionic, automotive), and together with recent trends such as Industrial Internet of Things (IIoT) and Fog/Edge computing, they are paving the way for the rising revolution of \textit{Industry 4.0} \cite{naha2018fog, iiot_survey,stavdas2022networked}. 
%%
%% poco chiaro, riscrivere
%% -- begin
This transformation includes \textit{software-defined}, flexible and moving control, communication, computation, and decision-making components, deployed across the boundaries of the central cloud and the network edge (i.e., the \textit{things}), closer to the location where data is generated. % to benefit from lower latencies. 
%%
%% -- end
%%
This revolution applies in a large spectrum of areas, from smart factories to energy infrastructures and process automation, which require smart devices featuring rich connectivity, local intelligence, and autonomous behavior \cite{shift2rail, windriveriot, hercules2020, 5gcity_H2020, hermann2016design, klingensmith2019using, klingensmith2018hermes}.

\gigi{aggiungere scenari d'uso reali per motivare orchestration su I4.0, vedere 30 e 34}

%%% %%% Challenges and requisiti per i nodi edge in I4.0
With this paradigm shift, IIoT and Fog/Edge computing must meet critical requirements like performance scalability, interoperability, low latency and agility, aimed at efficient deployment, reconfigurability and real-timeliness, in addition to mandatory regulatory requirements involving functional safety (IEC61508) and control (IEC61131). 
In these contexts, fog/edge computing systems are therefore treated as mixed-criticality systems\cite{burns2022mixed}, i.e., systems that allow embedding tasks (often real-time) at different criticality levels on the same hardware platform in an isolated manner. 

%% Virtualizzazione
%%
Virtualization is seen as a key technology since it provides support for resource partitioning and multiplexing, allowing the execution of heterogeneous Operating System (OS) (real-time and general-purpose) environments \cite{heiser2011virtualizing}, and becoming a prominent way for the industry to consolidate multiple software systems on the same system-on-a-chip (SoC) in a flexible way \cite{bloomberg_chip_shortage, blackberry_qnx_chip_shortage, cinque2021virtualizing}. 
%% -- ? riscrivere, non ho capito cosa si intendeva
%\mb{capoverso non chiaro, potenziale strip --}
%IoT/IIoT is inhabited by heterogeneous devices at edge level, including Multiprocessor System-on-Chip (MPSoC), with asymmetric multiprocessing (AMP) characteristics, dedicated hardware accelerators (e.g., FPGA, GPU), and rich I/O capabilities. Thus, there is also a trend in adopting hybrid virtualization solutions that try to address high portability and adaptability, with a rich set of I/O virtualization features. 
%% --

%% Container
%%
Lightweight virtualization solutions, such as containers, are gaining the limelight for the real-time and mixed-criticality scenarios mentioned above, since they promise to deliver low-latency, bandwidth-efficient, and resilient services with a reduced overhead and higher scalability compared to classical hypervisor-based solutions.\cite{morabito2018consolidate,struhar2020rtcontainerssurvey,abeni2019container, cinque2019rt, cinque2021preventing, goldschmidt2018container, tasci2018container, barletta2022achieving}. Moreover, containers are seamlessly integrated into orchestration mechanisms and platforms (e.g., Docker Swarm \cite{docker_swarm}, Kubernetes \cite{k8s}). On the other hand, OS-level virtualization is known to suffer from a reduced degree of isolation compared to hypervisor-based virtualization, and thus cannot be seen as a panacea \cite{randal2020ideal}.
%\mb{non riesco a far passare bene il concetto che un'orchestrazione per mixed-criticality deve obbligatoriamente passare per hypervisor-based containers per sfruttare i vantaggi di uno e dell'altro ----> l'orchestratore deve essere flessibile per poter incorporare le varie tecniche di virtualizzazione in maniera trasparente}

%% Orchestrazione
%%
\mb{esemplificare} With the spread of virtualized components, \textit{orchestration systems} have gained paramount importance %in the environment, 
since they automatically place, deploy, monitor and migrate the packaged software across the hardware infrastructure, behaving as cloud operating systems and controlling the whole system \cite{casalicchio2019container, khan2017key, rodriguez2019orchestration}. 
All this leads to the need for \textit{criticality-aware} orchestration solutions, able to cope with highly distributed ecosystem while providing the highest isolation guarantees to critical tasks, preventing severe faults/attacks within low-critical domains to interfere against high-critical ones, through the joint use of different virtualization technologies. The work in \cite{gogouvitis2020seamless} highlights that container orchestration is the key technology to unify different computing domains, although current orchestration systems provide no support for real-time applications. Similarly, in \cite{johansson22kubernetes} container orchestration is seen as a chance for improving the recovery performance in a distributed control system scenario. 

%% Orchestrazione real-time
Recently, several studies proposed Kubernetes-based solutions for real-time cloud computing orchestration \cite{fiori2022kube, johansson22kubernetes, toka2021ultra, struhar21react, eidenbenz2020latency}. 
%% Mancanze dell'orchestrazione rt
Despite the existing literature introducing the support for deploying real-time containers, orchestration for time predictable cloud is still at the dawn. Specifically, current solutions lack of determinism (e.g., time-sensitive placement and migration of resources), support for heterogeneous devices and their peculiarities (e.g., taking into account shared accelerators in deploy decisions), and capability of meeting the different degrees of isolation and assurance required by the workloads.

\gigi{riprendere il discorso virt hybrid (non solo container..)}
%Virtualization will be extensively used also in high-performance computing (HPC) platforms, which offer the power needed by the modern industrial systems and edge computing architectures by using devices like GPUs, FPGAs, and other kinds of accelerators. No solutions are available yet, capable to face such heterogeneous environments while guaranteeing easy porting, isolation, and real-time properties. Containers are a promising solution for these contexts, combining flexibility and scalability, but they are not mature yet for full adoption in industrial domains.

%% PROPOSAL
On this basis, we propose a novel model for real-time mixed-criticality container orchestration in edge systems, taking full advantage of heterogeneous virtualization technologies like OS-level virtualization and hypervisor-based containers to meet specified requirements. Specifically, our contributions fill the gap in the literature by providing: 
\begin{itemize}
%- Modello (assurance, reti multiple, criticità, timeliness, WCET diverso su nodi diversi)
%- Differenza dei comportamenti dei tipi nodo sotto carico
%- Metriche di monitoring
%- Differenza architetturale rispetto ai previous works: focus su eterogeneità di virtualizzazione
    \item An orchestration model for fog/edge cloud infrastructures that focuses on different assurance levels, time sensitive networks, and mixed-criticality real-time containers \gigi{including WCET analysis and time guarantees....check};
    \item A design architecture and a Kubernetes-based implementation of the proposed orchestration model, highlighting architectural differences against the state-of-the-art solutions;% (we focus on heterogeneous devices and virtualization technologies).
    \item \mb{check}An analysis of edge nodes behaviors under different stressful conditions;
    \item Monitoring metrics selection for accurately define and support the orchestration strategies.
\end{itemize}

The rest of the paper is organized as follows. \sectionautorefname{}~\ref{sec:related}  discusses related work. \sectionautorefname{}~\ref{sec:model} provides the system model for the orchestration of mixed-criticality fog/edge cloud infrastructure for Industry 4.0. \sectionautorefname{}~\ref{sec:architecture} %and \sectionautorefname{}~\ref{sec:implementation} 
describes the proposed architecture and the details of our Kubernetes-based implementation, respectively. \sectionautorefname{}~\ref{sec:results} provides an experimental analysis for proving the applicability of the proposed architecture. \sectionautorefname{}~\ref{sec:conclusion} concludes the paper.

